Simulation Studies of Charge Transport on Resistive Structures in Gaseous Ionization Detectors

We developed a tool for the simulation of charge transport on a conducting plate of finite dimensions. This tool is named Chani. Main motivation of developing Chani was to provide a tool for the optimization of the dimensions and resistivity of the anode electrodes in spark-protected Micropattern Gaseous Detectors (MPGD). In this thesis, we start with the general description of the LHC and the ATLAS Experiment. Then, we review the gaseous ionization detector technologies and in particular, the micromegas technology. We then present the working principles of Chani along with the example calculations. These examples include comparisons with the analytically solvable problems which shows that the simulation results are reasonable.

==> ch5.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\chapter{CONCLUSION}\label{ch:ifnecch4}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

A working simulator for the charge transport on rectangular surfaces is developed. It is possible to calculate the time needed for the total discharge and the spread of the charge over to surface using Chani. Although it is developed to help the design of the gaseous ionization detectors, Chani’s features can find applications in many fields where the understanding of charge transport properties is important. Specifically for particle detectors with resistive anodes, Chani can be used to guess the rate capabilities of the detectors from the discharge times and possible cross-talks between the readout strips due to the charge spread.


==> sembol.tex <==
\begin{tabular}{lrl}
{$\alpha$}              & : & Alpha  \\
{$\beta$}               & : & Beta \\
\end{tabular}

